Impact of hole-doping on the thermoelectric properties of pyrite FeS2

We present a comprehensive first-principles analysis of the thermoelectric transport properties of hole-doped pyrite FeS$_2$ that includes electron-phonon interactions. This work was motivated by the observed variations in the magnitude of thermopower reported in previous experimental and theoretical studies of hole-doped FeS$_2$ systems. Our calculations reveal that hole-doped FeS$_2$ exhibits large positive room-temperature thermopower across all doping levels, with a room-temperature thermopower of 608 $\mu$V/K at a low hole-doping concentration of 10$^{19}$ cm$^{-3}$. This promising thermopower finding prompted a comprehensive investigation of other key thermoelectric parameters governing the thermoelectric figure of merit $ZT$. The calculated electrical conductivity is modest and remains below 10$^5$ S/m at room-temperature for all doping levels, limiting the achievable power factor. Furthermore, the thermal conductivity is found to be phonon driven, with a high room-temperature lattice thermal conductivity of 40.5 W/mK. Consequently, the calculated $ZT$ remains below 0.1, suggesting that hole-doped FeS$_2$ may not a viable candidate for effective thermoelectric applications despite its promising thermopower.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\usepackage{caption}
\usepackage{indentfirst}

